Riemannian Dictionary Learning and Sparse Coding for Positive Definite Matrices

Data encoded as symmetric positive definite (SPD) matrices frequently arise in many areas of computer vision and machine learning. While these matrices form an open subset of the Euclidean space of symmetric matrices, viewing them through the lens of non-Euclidean Riemannian geometry often turns out to be better suited in capturing several desirable data properties. However, formulating classical machine learning algorithms within such a geometry is often non-trivial and computationally expensive. Inspired by the great success of dictionary learning and sparse coding for vector-valued data, our goal in this paper is to represent data in the form of SPD matrices as sparse conic combinations of SPD atoms from a learned dictionary via a Riemannian geometric approach. To that end, we formulate a novel Riemannian optimization objective for dictionary learning and sparse coding in which the representation loss is characterized via the affine invariant Riemannian metric. We also present a computationally simple algorithm for optimizing our model. Experiments on several computer vision datasets demonstrate superior classification and retrieval performance using our approach when compared to sparse coding via alternative non-Riemannian formulations.

==> jrnl_intro.tex <==
\section{Introduction}
\label{sec:intro}

Symmetric positive definite matrices---in the form of region covariances~\cite{porikli1}---play an important role as data descriptors in several  computer vision applications. Notable examples where they are used include object recognition~\cite{kernelsheartly2013}, face recognition~\cite{pang2008gabor}, human detection and tracking~\cite{porikli3,ma2012bicov}, visual surveillance~\cite{cherian2011dirichlet}, 3D object recognition~\cite{fehr2012compact}, among others. Compared with popular vectorial descriptors, such as bag-of-words, Fischer vectors, etc., the second-order structure that covariance matrices offer makes them particularly appealing. For instance, covariance descriptors offer a convenient platform for fusing multiple features into a compact form independent of the number of data points. By choosing appropriate features, this fusion can be made invariant to image affine distortions~\cite{ma2012affine}, or robust to static image noise and illumination variations, while generating these matrices remains efficient using integral image transforms~\cite{porikli3}.
%tosato2010multi

In this paper, we study SPD matrices in the context of sparse coding. The latter is now an important, established tool in signal processing and computer vision: it helps understand the inherent structure of the data~\cite{denoising2006,olshausen1997sparse}, leading to state-of-the-art results for a variety of vision applications~\cite{guha2012learning,wright2009robust,yang2009linear}. Given an input data point and an overcomplete dictionary of basis atoms, Euclidean sparse coding seeks a representation of this point as sparse linear combination of atoms so that a squared Euclidean loss is minimized. Formally, if $\dict$ is the dictionary and $\gdatapt$ the input data point, generic sparse coding may be formulated as
\begin{equation}
\nlmin_{\theta}\quad\loss(\gdatapt, \dict, \theta) + \lambda\sparse(\theta),
\label{eq:abstract_eqn}
\end{equation}
where the loss function $\loss$ measures reconstruction accuracy obtained by using the ``code'' $\theta$, while $\lambda$ regulates the impact of the sparsity penalty $\sparse(\theta)$.

Sparse coding has found great success for vector valued data, so it is natural to hope for similar benefits when applying it to the more complex setting of data represented via SPD matrices. However, applying sparse coding to SPD matrices is not straightforward, a difficulty that arises primarily because SPD matrices form a curved Riemannian manifold of negative sectional curvature (so that distances along the manifold are lower than corresponding Euclidean distances). As a result, this manifold cannot be isometrically embedded into Euclidean space through operations such as mere vectorization, without introducing embedding errors. Such errors can affect the application performance~\cite{pennec2006riemannian,porikli3}. On the other hand, computing distances and solving optimization problems on the SPD manifold is computationally demanding (see Section~\ref{sec:background}). Thus care must be taken to select an appropriate loss function. 

The main goal of this paper is to study sparse coding of SPD matrices in their native Riemannian geometric context by using a dictionary comprised of SPD matrices as atoms. Towards this end, we make the following contributions.
\begin{itemize}
\item \emph{Formulation:} We propose a novel model that finds nonnegative sparse linear combinations of SPD atoms from a given dictionary to well-approximate an input SPD matrix. The approximation quality is measured by the squared intrinsic Riemannian distance. As a  theoretical refinement to our model, we describe a surprising but intuitive geometric constraint under which the nonconvex Riemannian sparse coding task actually becomes convex.
\item \emph{Optimization:} The main challenge in using our formulation is its higher computational cost relative to Euclidean sparse coding. However, we describe a simple and effective approach for optimizing our objective function. 
\item \emph{Experiments:} We present results on a few computer vision tasks on several  state-of-the-art datasets to demonstrate superior performance obtained by using our new sparse coding model.  % compared with competing approaches.
\end{itemize}

To set the stage for presenting our contributions, we first survey some recent methods suggested for sparse coding. After that we review key tools from Riemannian geometry that we will use to develop our ideas. Throughout we work with real matrices. The space of $d\times d$ SPD matrices is denoted as $\spd{d}$, symmetric matrices by $\sym{d}$, and the space of (real) invertible matrices by $\genlinear(d)$. By $\Log(X)$, for $X\in\spd{}$, we mean the principal matrix logarithm.


==> jrnl_optimization.tex <==
\section{Optimization}
\label{sec:optimization}

TODO
